The Camassa-Holm equation as an incompressible Euler equation: a geometric point of view

The group of diffeomorphisms of a compact manifold endowed with the L^2 metric acting on the space of probability densities gives a unifying framework for the incompressible Euler equation and the theory of optimal mass transport. Recently, several authors have extended optimal transport to the space of positive Radon measures where the Wasserstein-Fisher-Rao distance is a natural extension of the classical L^2-Wasserstein distance. In this paper, we show a similar relation between this unbalanced optimal transport problem and the Hdiv right-invariant metric on the group of diffeomorphisms, which corresponds to the Camassa-Holm (CH) equation in one dimension. On the optimal transport side, we prove a polar factorization theorem on the automorphism group of half-densities.Geometrically, our point of view provides an isometric embedding of the group of diffeomorphisms endowed with this right-invariant metric in the automorphisms group of the fiber bundle of half densities endowed with an L^2 type of cone metric. This leads to a new formulation of the (generalized) CH equation as a geodesic equation on an isotropy subgroup of this automorphisms group; On S1, solutions to the standard CH thus give particular solutions of the incompressible Euler equation on a group of homeomorphisms of R^2 which preserve a radial density that has a singularity at 0. An other application consists in proving that smooth solutions of the Euler-Arnold equation for the Hdiv right-invariant metric are length minimizing geodesics for sufficiently short times.

==> sec-Euler-Arnold_rer.tex <==
%!TEX root =  ./Final.tex

\section{The $H^{\Div}$ right-invariant metric on the diffeomorphism group}
\label{Sec:EulerArnold}

In this section, we summarize known results on the $H^{\Div}$ right-invariant metric on the diffeomorphism group. 
We now define the $H^{\Div}$ right-invariant metric
\begin{definition}\label{DefinitionHdiv}
Let $(M,g)$ be a Riemannian manifold and $\on{Diff}^s(M)$ be the group of diffeomorphisms which belong to $H^s(M)$ for $s > d/2 + 1$. The right-invariant $H^{\Div}$ metric, implicitely dependent on two positive real parameters $a,b$, is defined by
\begin{equation}\label{Eq:Metric}
G_\varphi(X_\varphi,X_\varphi) = \int_M a^2| X_\varphi \circ \varphi^{-1} |^2 + b^2\Div(X_\varphi \circ \varphi^{-1})^2 \ud \! \on{vol} \,.
\end{equation}
\end{definition}
The Euler-Arnold equation in one dimension (that is on the circle $S^1$ for instance) is the well-known Camassa-Holm equation (actually when $a=b=1$):
\begin{equation} \label{Eq:CH}
a^2\partial_{t} u - b^2\partial_{txx} u  +3 a^2\partial_{x} u \,u  - 2b^2\partial_{xx} u \,\partial_x u - b^2\partial_{xxx} u \,u = 0\,.
\end{equation}
On a general Riemannian manifold $(M,g)$, the equation can be written as, with $n = a^2 u^\flat  + b^2 \ud \delta u^\flat$,
\begin{equation}\label{Eq:HdivGeometricForm}
\partial_t n + a^2\left(\Div(u) u^\flat +  \ud \langle u , u \rangle + \iota_u \ud u^\flat\right)  + b^2\left( \Div(u) \ud \delta u^\flat + \ud \iota_u \ud \delta u^\flat\right) = 0\,,
\end{equation}
where the notation $\flat$ corresponds to lowering the indices. More precisely, if $u \in \chi(M)$ then $u^\flat$ is the $1$-form defined by $v \mapsto g(u,v)$. The notation $\delta$ is the formal adjoint to the exterior derivative $\ud$ and $\iota$ is the insertion of vector fields which applies to forms.

\par \textbf{On the well-posedness of the initial value problem.} Although the theorem below is not stated in this particular form in \cite{Ebin1970}, this result can be seen as a byproduct of their results as explained in \cite[Theorem 4.1]{MisolekPreston2010}. For similar smoothness results in the case of smooth diffeomorphisms, we refer the reader to \cite[Theorem 3]{Constantin2003}.
\begin{theorem}\label{Th:EbinMarsden}
 On $\on{Diff}^s(S_1)$ for $s \geq 2$ integer, the $H^{1}$ right-invariant metric is a smooth and weak Riemannian metric. Moreover, if $s\geq 3$, the exponential map is a smooth local diffeomorphism on $T\on{Diff}^s(S_1)$.
\end{theorem}
Global well-posedness does not hold in one dimension since there exists smooth initial conditions for the Camassa-Holm equation such that the solutions blow up in finite time.

In higher dimensions, the initial value problem has been studied by Michor and Mumford \cite[Theorem 3]{MumfordMichorHdiv}. This is not a direct result of \cite{Ebin1970} since the differential operator associated to the metric is not elliptic. They prove that the initial value problem on the space of vector fields is locally well posed for initial data in a Sobolev space of high enough order. Although the proof could probably be adapted to the case of a Riemannian manifold, in that case, the result of local well posedness is not proven yet. 

\par \textbf{On the metric properties of the  $H^{\Div}$ right-invariant metric.}
Michor and Mumford already had the following non-degeneracy result in \cite{Michor2005}.
\begin{theorem}[Michor and Mumford]\label{Th:MM}
The distance on $\on{Diff}(M)$ induced by the $H^{\Div}$ right-invariant metric is non-degenerate. Namely, between two distinct diffeomorphisms the infimum of the lengths of the paths joining them is strictly positive.
\end{theorem}
Due to the presence of blow up in the Camassa-Holm equation, metric completeness does not hold since it would imply geodesic completeness, that is global well posedness. However, it is still meaningful to ask whether geodesics are length minimizing for short times. Since the Gauss lemma is valid in a strong $H^s$ topology, this ensures that geodesics are length minimizing among all curves that stay in a $H^s$ neighborhood, see also \cite{Constantin2003}.
However, this is \emph{not} enough to prove that the associated geodesic distance is non degenerate since an almost minimizing geodesic can escape this neighborhood for arbitrarily small energy. This is what happens for the right-invariant metric $H^{1/2}$ on the circle $S_1$ where the metric is degenerate although there exists a smooth exponential map similarly to our case, see \cite{Escher12}.





==> sec-Unbalanced-optimal-transport.tex <==


\section{The corresponding Monge formulation}\label{Sec:Monge}
By the geometric point of view developed above, it is possible to derive a Monge formulation directly and also to derive a pre-formulation of the Monge-Ampère equation. We first derive formally the equations for which a precise meaning will be given in the next sections. \subsection{The Monge formulation}
The first important consequence of the $L^2$ metric on the group and the Riemannian submersion is that one can define a Monge formulation of the Wasserstein-Fisher-Rao metric as follows:
\begin{equation}\label{Eq:MongeFormulation}
\on{WF}(\rho_0, \rho_1) = \inf_{(\varphi,\lambda) } \left\{ \| (\varphi,\lambda) - (\Id,1)  \|_{L^2(\rho_0)} \, : \, \varphi_*(\lambda^2 \rho_0 )= \rho_1 \right\}\,.
\end{equation}
It is then possible to derive a pre-formulation to the classical Monge-Ampère equation at least formally: 
Under the assumption that there exists a smooth minimizer $(\varphi,\lambda)$ of \eqref{Eq:MongeFormulation}, there exists a function $p \in C^\infty(M,\R)$ given by the Lagrange multiplier rule such that
\begin{equation}\label{Eq:MongeFormulation2}
(\varphi(x),\lambda(x)) = \exp_{(x,1)}^{\mathcal{C}(M)}\left(-\frac 12 \nabla p(x),-p(x)\right)\,,
\end{equation}
where $\exp_{(x,1)}$ denotes the Riemannian exponential map on $\mathcal{C}(M)$. The "pushforward" constraint now reads
\begin{equation}
(|1-p(x)|^2 + \frac 14\|\nabla p(x)\|^2) \rho_0(x) =\on{Jac}( \varphi)(x)\, \rho_1(\varphi(x))\, 
\end{equation}
where $$\varphi(x) = \exp^{M}_x\left(-\arctan\left(\frac{\|\nabla p(x)\|}{2(1\comment{-}p(x))}\right) \frac{\nabla p(x)}{\|\nabla p(x)\|}\right)\,.$$
Under the change of variable $z \eqdef - \log(1-p)$, the previous equations become
\begin{equation}
(1 + \frac14 \|\nabla z\|^2) e^{-2z} \rho_0 = \det(D \varphi) \rho_1\circ \varphi \, 
\end{equation}
and $$\varphi(x) = \exp^{M}_x\left(-\arctan\left(\frac{1}{2} \|\nabla z \| \right) \frac{\nabla z(x)}{\|\nabla z(x)\|}\right)\,.$$
However, the function $p$ (or $z$) is not completely characterized. Indeed, in standard optimal transport, the optimal potential is convex. Convexity will be replaced by $c$-concavity for a particular cost. 
Note that this result has been established in the Euclidean case in  \cite[Theorem 6.7]{LieroMielkeSavareLong} under mild assumptions on the densities. Their result is based on a detailed study of the equivalent Kantorovich formulation which is presented in \ref{Sec:KantorovichFormulation}. This equivalent formulation is only proven in \cite{LieroMielkeSavareLong} and \cite{GeneralizedOT2} in the Euclidean case and it is expected to be true \cite[Section 8.5]{LieroMielkeSavareLong} in the Riemannian case. %Moreover, once this equivalence is proven in the Riemannian case, an adaptation of  \cite[Theorem 6.7]{LieroMielkeSavareLong} is still needed. 
%\par
%In the next section, we present the Kantorovich formulation associated with the Monge formulation and we prove the equality between the Kantorovich and the dynamic formulations of the $\on{WF}$ metric. 


%\subsection{The Kantorovich Formulation} \label{Sec:KantorovichFormulation}
%From a variational point of view, it is important to derive a relaxation of the Monge formulation.
%It is of interest to understand first the simple situation when the source and target measures are single Dirac masses and when $M$ is a convex and compact domain in the Euclidean space as studied in \cite{GeneralizedOT1}. This also applies to the case of a Riemannian manifold since it can be shown using the static formulation proven in this section.
%\begin{proposition}
%Let $M$ be a convex and compact domain in $\R^d$ with the Euclidean metric.
%Let $m_1\delta_{x_1}$ and $m_2\delta_{x_2}$ be two Dirac masses with $x_1,x_2 \in M$ and $m_1,m_2 \in \R_+^*$. 
%
%If $d(x_1,x_2) < \pi/2$, there exists a unique geodesic which is $m(t) \delta_{x(t)}$ where $(x(t),m(t))$ is the geodesic in $M\times \R_+^*$ with the cone metric between $(x_1,m_1)$ and $(x_2,m_2)$.
%
%If $d(x_1,x_2) > \pi/2$, there exists a unique geodesic which is $m_1(t) \delta_{x_1} + m_2(t)\delta_{x_2}$ where $m_1(t) = m_1 (1-t)^2$ and $m_2(t) = m_2 t^2$ describe the geodesics between $(x_i,m_i)$ and the cone point for $i= 1,2$.
%
%If $d(x_1,x_2) =\pi/2$, there exists an infinite number of geodesics which are convex combinations of the two first types defined above.
%\end{proposition}
%
%The important point is that passing to the case of measures the angle of the cone has been divided by $2$.
%This is because the optimization problem is not formulated on the space of geodesics on $M\times \R_+^*$, but on the space of measures on $M$. And, in particular, the cost between Dirac masses has to be convex.
%\par
%The generalization to any positive Radon measures of the Kantorovich relaxation requires the definition of a convex functional which is one-homogeneous on the space of Radon measures described below. The next theorem is proven in \cite{GeneralizedOT2} and in another form in \cite{LieroMielkeSavareLong}, both only in the Euclidean case. We now extend it to in a Riemannian setting.
%\begin{theorem}\label{Th:DynamicToStaticOnRiemannianManifolds}
%For two given positive Radon measures $\rho_1,\rho_2$, we define, for $\mathcal{M}_+(M^2)$ the space of positive Radon measures on $M^2$,
%\begin{align}
%		\Gamma(\rho_1,\rho_2) \eqdef \left\{
%			(\gamma_1,\gamma_2) \in \big(\mathcal{M}_+(M^2)\big)^2 \colon
%			p^1_* \gamma_1 = \rho_1,\, p^2_* \gamma_2 = \rho_2
%			\right\}\,,
%	\end{align}
%	where $p^1$ and $p^2$ denote the projection on the first and second factors of the product $M^2$.
%The variational problem associated with the Wasserstein-Fisher-Rao distance is
%\begin{align}
%	\label{Eq:StaticProblem}
%		\on{WF}^2(\rho_1,\rho_2)  = \min_{(\gamma_1,\gamma_2) \in \Gamma(\rho_1,\rho_2)}
%			\int_{M^2} d_{\mathcal{C}(M)}^2 \left((x,\frac{\ud \gamma_1}{ \ud \gamma}),(y,\frac{\ud \gamma_2}{ \ud \gamma})\right) \ud \gamma(x,y) \,,
%	\end{align}
%where $d_{\mathcal{C}(M)}^2$ is the square of the cone distance given in definition \ref{def:Cone} and $\gamma$ is any measure that dominates $\rho_1$ and $\rho_2$. 
%\end{theorem}
%
%\begin{proof}
%The proof is given in Appendix \ref{Sec:OtherProofs}.
%\end{proof}
%
%\begin{remark}
%The fact that $S(\gamma_1,\gamma_2) \eqdef \int_{M^2} d_{\mathcal{C}(M)}^2 \left((x,\frac{\ud \gamma_1}{ \ud \gamma}),(y,\frac{\ud \gamma_2}{ \ud \gamma})\right) \ud \gamma(x,y)$ is well defined follows from the application of \cite[Theorem 5]{rockafellar1971integrals}. It does not depend on the choice of the measure $\gamma$ since the function $d^2$ is one-homogeneous w.r.t. the mass variables. As a consequence of Rockafellar's theorem \cite[Theorem 5]{rockafellar1971integrals}, $S$ is convex and lower-semicontinuous on the space of Radon measures as the Legendre-Fenchel transform of a convex functional on the space of continuous functions.
%\end{remark}
%We also state without proof the dual formulation which is given by the application of Fenchel-Rockafellar duality theorem, see \cite{GeneralizedOT2}.
%
%\begin{proposition}\label{Th:Duality}
%It holds
%\begin{equation}
%\on{WF}^2(\rho_0,\rho_1) =
% \sup_{(\phi,\psi)\in C(M)^2  }  \int_M \phi(x) \ud \rho_0(x) + \int_M \psi(y) \ud \rho_1(y) \\
%\end{equation}
%subject to $\forall (x,y)\in M^2$,
%\begin{equation}
%\begin{cases}\label{MultiplicativeConstraint}
% \phi(x) \leq 1\,, \quad \psi(y) \leq 1\, , \\
%(1-\phi(x))(1-\psi(y)) \geq \cos^2\left(d(x,y)\wedge {(\pi / 2)}\right)\,.
%\end{cases}
%\end{equation}
%A reformulation of this linear optimization problem is
%\begin{equation}\label{Eq:Reformulation}
%\on{WF}^2(\rho_0,\rho_1) =
% \sup_{(z_0,z_1)\in C(M)^2  }  \int_M 1-e^{-z_0(x)} \ud \rho_0(x) + \int_M 1-e^{-z_1(y)} \ud \rho_1(y) 
%\end{equation}
%subject to $\forall (x,y)\in M^2$,
%\begin{equation}\label{Eq:Constraint}
%z_0(x)+ z_1(y) \leq -\log\left(\cos^2\left(d(x,y)\wedge {(\pi / 2)}\right)\right)\,.
%\end{equation}
%\end{proposition}
%
%Interestingly, the last formulation can be further reduced since the exponential $r \mapsto e^{r}$ is the Fenchel-Legendre conjugate associated with the Kullback-Leibler divergence defined below. Therefore, using duality again, it is proven in \cite{LieroMielkeSavareLong} that the static problem in Proposition \ref{Th:Duality} can be rewritten as
%\begin{multline}\label{Eq:KLFormulation}
%\on{WF}^2(\rho_0,\rho_1) = \inf_{\gamma \in \mathcal{M}_+(M^2)}\on{KL}(\Proj^1_*\gamma,\rho_0) + \on{KL}(\Proj^2_* \gamma,\rho_1) \\ - \int_{M^2} \log(\cos^2(d(x,y) \wedge {(\pi / 2)})) \ud \gamma(x,y)
%\end{multline}
%with 
%$$ \on{KL}(\mu, \nu) = \int \frac{\ud \mu}{\ud \nu} \log\left(\frac{\ud \mu}{\ud \nu}\right) \ud \nu + |\nu| - |\mu|  \,,$$
%the Kullback-Leibler divergence. Formulation \eqref{Eq:KLFormulation} of unbalanced optimal transport and its extensions have been intensively developed in \cite{LieroMielkeSavareLong}, where generalizations of this metric are studied in spaces such as Hausdorff topological spaces endowed with a (pseudo) distance satisfying mild conditions. More interestingly, in our situation where the underlying space $M$ is a finite dimensional Riemannian manifold, is the existence of solutions to the dual problem \eqref{Eq:Reformulation} - \eqref{Eq:Constraint}, which is proven in \cite{LieroMielkeSavareLong}. In particular, we rely on the existence results given in \cite[Section 6.2]{LieroMielkeSavareLong} in a larger class of potentials than simply continuous. We also strongly rely on their characterization presented in \cite[Theorem 6.3]{LieroMielkeSavareLong}.
%
%
%
%\subsection{Polar factorization on the automorphism group of half-densities and Monge-Ampère equation}
%One can state a similar version to Brenier's polar factorization theorem \cite{Brenier1991} in this context. Actually, this can be understood as a constrained version of the polar factorization, since the diffeomorphisms are restricted to be  automorphisms. To the best of our knowledge, this is not a direct consequence of \cite{McCann2001} or \cite{LieroMielkeSavareLong}. 
%However, adapting arguments from these two articles, under mild conditions on the initial and final densities, we give a rigorous meaning to the equivalent of the Monge-Amp\`ere equation and we propose a polar factorization on the automorphism group of the cone. 
%
%We use define a c-concave function as in \cite{McCann2001}.
%
%\begin{definition} \label{ def-cconcave}
%A function $z$: $M \to \R\cup{ \left\{ \pm \infty \right\}} $ is said to be c-concave if there exists $\bar z$: $M \to \R\cup{ \left\{ \pm \infty \right\}} $ such that 
%
%\begin{equation}\label{Eq:Constraint}
%z(x) = \inf_{y\in  M} \left[ c(x,y) - \bar z(y) \right], \quad \forall x \in M.
%\end{equation}
%\end{definition}
%
%\begin{definition}[Admissible measures]\label{Th:AdmissibleMeasures}
%We say that a positive Radon measure $\rho$ on $M$ is admissible (with respect to $\on{vol}$) if for any $x \in M$, there exists $y \in \on{Supp}(\rho)$ such that $d(x,y)<\pi /2$.
%\end{definition}
%Note that when the diameter of $M$ is less than $\pi/2$ then all but the null measure are admissible.
%In general, when the null measure is considered, the geodesic is unique and is the geodesic corresponding to the Hellinger distance.
%To shorten the notations, we denote by $c$ the function $c(x,y) = -\log\left(\cos^2\left(d(x,y)\wedge {(\pi / 2)}\right)\right)$ which intervenes in the constraint \eqref{Eq:Constraint} of the dual formulation. We prove that a solution of $\on{WF}$, in the form \eqref{Eq:Reformulation} - \eqref{Eq:Constraint} leads to a solution of the associated Monge problem defined by \eqref{Eq:MongeFormulation}. %The method of the proof is similar to the classical case of optimal transport with minor adaptions due to the cost. 
%
%
%\input{sec-ppolaire}
%



==> sec-ppolaire-bis.tex <==
%!TEX root = ./WFR to Hdiv2.tex

\begin{lemma}[sub-differentiability] \label{subdiff}
%\begin{itemize}
%\item Let $y \in M$, the function $f$ defined on $M$ by $f(x)= -\ln(\cos^2(d (x,y ))$ is super-differentiable.
%\item Let $y \in M $, the function $g$ defined on $M$ by $g(x)= -\ln(\cos^2(d^2_{\frac{\pi}{2}}(x,y))$ is super-differentiable on $B_d{(y,\frac{\pi}{2})}$.
%\end{itemize}
 Let $y \in M $, the function $g$ defined on $M$ by $g(x)= \cos^2\left(d (x,y)\right)$ is sub-differentiable.
\end{lemma}
\begin{proof}
The function  $ d^2(\cdot,y)$ is super-differentiable see \cite[Proposition 6]{McCann2001} for instance. Therefore $d^2_{{\pi}/{2}}(\cdot,y)=\left(d(x,y)\wedge {(\pi / 2)}\right)$ %\on{inf}\left(d^2(\cdot,y), \frac{\pi}{2}\right)$
is also super-differentiable and %Since the function $-\log\left(\cos^2(\sqrt{2\cdot}\right))$ is $C^1$ on $[0,\frac{\pi}{2}[$ 
the function $g$ is sub-differentiable as the combinaison of a decreasing $C^1$ function and the super-differentiable function  $ d^2_{{\pi}/{2}}(\cdot,y)$, see \cite[Lemma 5]{McCann2001}. 
\end{proof}

\begin{proposition}[Approximate differentiability and optimality]\label{prop:approx}
Let $\rho_0$, $\rho_1$ be two positive Radon measures and $(z_0, z_1)$ be the generalized optimal potentials for $\on{WF}^2(\rho_0,\rho_1)$.  
Suppose that $\rho_0$ and $\rho_1$ are admissible and $\rho_0 << \on{vol}$, then $z_0$ is $\rho_0$ a.e. unique and approximate differentiable on $Supp(\rho_0)$. The optimal plan $\gamma$ in the formulation \eqref{Eq:KLFormulation} is unique, with marginals $\gamma_0=e^{-z_0}\rho_0$, $\gamma_1=e^{-z_1}\rho_1$ and concentrated on the graph of  
\begin{equation}\label{eq:unicitetransport}
x\mapsto \varphi(x)  =  \exp_x^M \left(-\arctan \left(\frac{\| \tilde \nabla z_0(\bar x)\|}{2}\right)   \frac{\tilde \nabla z_0(\bar x) }{\| \tilde \nabla z_0(\bar x)\| }\right),
\end{equation}
that is $\varphi_*\gamma_0=\gamma_1$ and $\gamma = ( \on{Id}\times \varphi )_{*} \gamma_0$. Finally
\begin{equation}\label{eq:optimalite}
\on{WF}^2(\rho_0,\rho_1)=  \int_M 1-e^{-z_0(x)} \ud \rho_0(x) + \int_M 1-e^{-z_1(y)} \ud \rho_1(y)\,.
\end{equation}
\end{proposition}
%\begin{corollary}
%Let $\rho_0$, $\rho_1$ be two admissibles radon measures, $(z_0, z_1)$ be the optimal potentials for $\on{WF}^2(\rho_0,\rho_1)$ then $\varphi$ is unique $\rho_0$ a.e.
%\end{corollary}
Note that $(z_0, z_1)$ may not be admissible in \eqref{Eq:Reformulation} but \eqref{eq:optimalite} still holds true. The proof of this proposition (being more technical) is given in Appendix \ref{Sec:OtherProofs}, we prefer to discuss the corresponding formulation of the Monge-Amp\`ere equation hereafter.
\par
Following Brenier's approach in the case of optimal transport, see \cite[Section 1.4]{Brenier1991} and \cite[Section 12]{villani2008optimal}, we expect the potential found in Proposition \ref{prop:approx}, denoted by $z$, to be a solution of a Monge-Amp\`ere equation. To formally derive the equation we suppose that $z$ is smooth. Recall that 
$c(x,y)=-\log(\cos^2(d_{{\pi}/{2}}(x,y)))$ and $\varphi(x)= \exp^{M}_x\left(-\arctan\left(\frac{1}{2} \| \nabla z(x) \| \right) \frac{ \nabla z(x)}{\| \nabla z(x)\|}\right) $, therefore
$$
 2 \sqrt{2} \tan( d_{{\pi}/{2}} ( x , y)) \frac{\sqrt{2}}{2d_{{\pi}/{2}} (\bar x ,\bar y)}\nabla \left( {\frac12 d^2_{{\pi}/{2}} (\bar x,\bar y) }\right)=(\nabla_x c) (x,\varphi(x))
$$
and the sub-differentiable equality \eqref{MA} reads
\begin{equation}\label{MA2}
  \nabla z (x)-(\nabla_x c) (x,\varphi(x)) =0\,.
\end{equation}
Differentiating \eqref{MA2} and taking the determinant yields
\begin{equation}\label{MA3}
\det\left[ -\nabla^2 z(x) +(\nabla_{xx}^2 c)(x,\varphi(x))\right]= \left|\det \left[ (\nabla_{x,y} c)(x,\varphi(x)) \right] \right| \left| \det( \nabla \varphi)\right|.
\end{equation}
Notice that the c-convexity property of $z$ implies that $ -\nabla^2 z +(\nabla_{xx}^2 c)(x,\varphi(x))$ is a nonnegative symmetric matrice. To obtain the equation on $z$, we observe that $\varphi_*\left((1 + \frac14 \| \nabla z\|^2) e^{-2z} \rho_0\right) = \rho_1$ (see the proof of Proposition \ref{Th:PolarFactorisationStep} below for details) or equivalently 
$$
\left| \det( \nabla \varphi)\right| = e^{-2z }\left( 1 +  \frac14 \| \nabla z \|^2  \right) \frac{f}{g\circ \varphi }\,,
$$
for smooth $z$ and smooth positive measures $\rho_0$ and $\rho_1$ with densities $f$ and $g$ with respect to the volume measure $\on{vol}$.
Together with \eqref{MA3}, we obtain the $\on{WF}$-Monge-Amp\`ere equation 
defined by 
\begin{equation}\label{MA4}
\det\left[ -\nabla^2 z(x) +(\nabla_{xx}^2 c)(x,\varphi(x))\right]= \left|\det \left[ (\nabla_{x,y} c)(x,\varphi(x)) \right] \right| e^{-2z(x) }\left( 1 +  \frac14 \| \nabla z(x) \|^2  \right) \frac{f(x)}{g\circ \varphi(x) }\,,
\end{equation}
where $\varphi$ is given by \eqref{defphi} and satisfies the second boundary value problem: $\varphi$ maps the support of $\rho_0$ to the support of $\rho_1$. 
Following Brenier \cite[Section 1.4]{Brenier1991}, Proposition \ref{Th:PolarFactorisationStep} below can be taken as a definition of weak solutions for  the 
$\on{WF}$-Monge-Amp\`ere equation with second boundary value problem.
The question of regularity for the potential $z$ solution of a $\on{WF}$-Monge-Amp\`ere equation will be studied elsewhere. One would first need to compute the Ma-Trudinger-Wang tensor associated to $c$ see  \cite{figallide}, \cite[Section 12]{villani2008optimal}.
\begin{remark}
In optimal transport, the notation $\cexp_x(v)= \left[(-\nabla_x c) (x,\cdot)\right]^{-1}(v) $ is classical. Using this notation one remarks that \eqref{MA2} implies
$$
\varphi(x)=\cexp (-\nabla z(x)).
$$
\end{remark}
\begin{proposition}[Brenier's weak solution of $\on{WF}$-Monge-Amp\`ere]\label{Th:PolarFactorisationStep}
Let $\rho_0,\rho_1$ be two admissible measures such that $\rho_0$ has density w.r.t. the volume measure on $M$. Then, there exists a  $\rho_0$ a.e. unique  $c$-convex function on $M$, $z$, approximatively differentiable $\rho_0$-a.e., such that the associated unbalanced transport couple $(\varphi,\lambda)$ defined by
\begin{equation}\label{defphi}
\varphi(x) = \exp^{M}_x\left(-\arctan\left(\frac{1}{2} \|\tilde \nabla z(x) \| \right) \frac{\tilde \nabla z(x)}{\|\tilde \nabla z(x)\|}\right)\,
\end{equation}
and
\begin{equation}\label{deflambdai}
\lambda(x) = e^{-z(x)} \sqrt{1 + \frac14\| \tilde \nabla z(x) \|^2}
\end{equation}
satisfies 
\begin{equation}\label{Eq:MAEquation}
\pi[(\varphi,\lambda),\rho_0]=\varphi_*\left(\lambda^2 \rho_0\right)=\varphi_*\left((1 + \frac14 \|\tilde \nabla z\|^2) e^{-2z} \rho_0\right) = \rho_1\,.
\end{equation}
Moreover, $(\varphi,\lambda)$ is the unique $\rho_0$ a.e. unbalanced transport couple associated to a c-convex potential,also unique, such that $\pi[(\varphi,\lambda),\rho_0]= \rho_1 $. 
The potential $z$ is a weak solution for  the 
$\on{WF}$-Monge-Amp\`ere equation \eqref{MA4} with second boundary value problem and is characterized by  
\begin{equation}\label{eq:optimalite2}
\on{WF}^2(\rho_0,\rho_1)=  \int_M 1-e^{-z(x)} \ud \rho_0(x) + \int_M 1-e^{-z^c(y)} \ud \rho_1(y)\,.
\end{equation}
\end{proposition}
\begin{proof}
Let $(z_0, z_1)$ be the optimal potentials for $\on{WF}^2(\rho_0,\rho_1)$. From Proposition \ref{prop:approx}, we know that $ x \mapsto \varphi(x)=\exp^M_{ x}\left(-\arctan \left(\frac{\| \tilde \nabla z_0( x)\|}{2}\right)   \frac{\tilde \nabla z_0( x) }{\| \tilde \nabla z_0( x)\| }\right)$ is well defined $\rho_0$ a.e. and 
$\varphi_*(\gamma_0)=\gamma_1$ where $\gamma_i=\sigma_i \rho_i =e^{-z_i} \rho_i $, $i=0,1$. Therefore
\begin{align*}
\rho_1 &=\sigma_1^{-1}  \gamma_1= \sigma_1^{-1} \varphi_*(\gamma_0) =\sigma_1^{-1} \varphi_*\left(\sigma_0 \rho_0\right) \\
 &=  \varphi_*\left( e^{-z_0} \sigma_1^{-1} \circ \varphi  \rho_0\right) = \varphi_*\left( e^{-z_0} e^{z_1\circ \varphi } \rho_0\right)= \varphi_*\left( e^{-z_0} e^{ c(\cdot,\varphi(\cdot))} e^{-z_0}   \rho_0\right) \\
 &=  \varphi_*\left( e^{-2z_0}\left( 1 +  \frac14 \| \tilde \nabla z_0 \|^2  \right) \rho_0 \right)= \varphi_*\left(\left(e^{-z_0} \sqrt{1 + \frac14 \|\tilde \nabla z_0 \|^2} \right)^2  \rho_0\right)\\
 & =\pi\left[ \left( \varphi ,e^{-z_0} \sqrt{1 + \frac14\|\tilde \nabla z_0 \|^2} \right),\rho_0\right].%=\pi_{\rho_0} \left( \varphi ,e^{z_0} \sqrt{1 + \| \nabla z_0(x) \|^2} \right).
\end{align*}
We used that $\rho_0$ a.e.  $z_0(x)+z_1(\varphi(x))=c(x,\varphi(x)) $, $1 + \tan^2(x) = 1/\cos^2(x)$ and thus $1 + \frac14 \| \tilde \nabla z_0(x) \|^2 = e^{c(x,\varphi(x))}\,$. 
Equation \eqref{eq:optimalite}  is exactly \eqref{eq:optimalite2}.

To prove uniqueness, consider $z$ to be a c-convex function, such that $(\varphi,\lambda)$ are well defined through \eqref{defphi} and \eqref{Eq:MAEquation} and 
$\pi[(\varphi,\lambda),\rho_0]=\rho_1$. Then, we claim that $ \gamma = [\on{Id}\times \varphi]_* (e^{-z} \rho_0)$ is an optimal plan for  $\on{WF}^2(\rho_0,\rho_1)$ in \eqref{Eq:KLFormulation}. Indeed, let us check that $\gamma$ satisfies the optimality conditions of \cite[Theorem 6.3(b)]{LieroMielkeSavareLong}. 
\begin{itemize}
\item $\gamma$ is concentrated on the set of equality for a pair $(z,z^c)$ of c-convex functions.
By definition of $\varphi$, it holds $\rho_0$ a.e. and therefore $\gamma_0=e^{-z} \rho_0$ a.e.
\begin{equation}\label{cara}
z(x)+z^c(\varphi(x))= c(x,\varphi(x))\,. 
\end{equation}
Thus, $(z,z^c)$ satisfies for all $(x,y) \in M\times M$, $ z(x)+z^c(y) \leq c(x,y)$ with equality $\gamma$ a.e.
\item The marginals are absolutely continuos with respect to $\rho_0$ and $\rho_1$. It holds true for $\gamma_0=e^{-z} \rho_0$. 
Notice then that $ \rho_0$ a.e.
$$
\lambda^2(x)=e^{-2z(x)} (1 + \frac14\| \tilde \nabla z(x) \|^2)= e^{-z(x)}  e^{z^c(\varphi(x))}\,.
$$
It yields 
$$
\rho_1= \varphi_*(\lambda^2\rho_0)=  \varphi_*(   e^{z^c(\varphi(x))} e^{-z(x)} \rho_0)=e^{z^c} \varphi_*(   \gamma_0)= e^{z^c} \gamma_1\,,
$$
thus $\gamma_1= e^{-z^c}\rho_1$ and $\gamma$ is optimal for $\on{WF}^2(\rho_0,\rho_1)$. 
\end{itemize}
The computation \eqref{egalitepotentiel} yields \eqref{eq:optimalite2} and the uniqueness of the generalized optimal potentials for $\on{WF}^2(\rho_0,\rho_1)$ in Proposition \eqref{prop:approx} implies the uniqueness of $(z,\varphi,\lambda)$.

%The last equality is exactly \ref{Eq:MAEquation} in a weak sense. 
\end{proof}
Note that if $z$ is smooth, it satisfies \eqref{MA4}.
%An other proof of this fact is given in Appendix following the perturbation argument in \cite{McCann2001}. The alternative proof has the advantage to not suppose the existence of an optimal transport plan $\gamma$. 
It turns out that this factorization can be extended to a larger class containing the automorphism group of the cone $\on{Aut}(\mathcal{C}(M))$. In the following, we state a polar factorization theorem for a class of maps from $M$ to $C(M)$. We start with definitions.  % on measures such that the corresponding function $p$ in formulation \eqref{Eq:MongeFormulation2} only takes finite values and is approximately differentiable.
\begin{definition}
We define the generalized automorphism semigroup of $C(M)$ as the set of mesurable maps $\left(\varphi,\lambda \right)$ from $M$ to $C(M)$
\begin{equation}
\autgc (\mathcal{C}(M)) = \left\{ \left(\varphi,\lambda \right) \in \Mes(M,M)\ltimes \Mes(M,\R_+^*)  \right\}\,,
\end{equation}
endowed with the semigroup law
\begin{equation*}
(\varphi_1,\lambda_1) \cdot (\varphi_2,\lambda_2) = (\varphi_1 \circ \varphi_2,  (\lambda_1 \circ \varphi_2)  \lambda_2 )\,.
\end{equation*}
%We set 
%\begin{equation}
%\autgc (\mathcal{C}(M)) = \cup_{\rho_0 \in \mathcal{M}(M)  } \autg (\mathcal{C}(M)).
%\end{equation}
%For any Radon measure $\rho_0$, 
We also consider the stabilizer of the volume measure in the automorphisms of $C(M)$. It is a subsemigroup and is defined by 
\begin{equation}
\autgc_{\on{vol}} (\mathcal{C}(M)) = \left\{ \left(s,\lambda \right) \in \autgc (\mathcal{C}(M)) \,:\, \pi\left((s,\lambda),\on{vol}\right)=\on{vol}  \right\}\,.
\end{equation}
By abuse of notation, any $\left(s,\lambda \right) \in \autgc_{\on{vol}} (\mathcal{C}(M))$ will be denoted  $\left( s, \sqrt{\on{Jac}(s)} \right)$ meaning that for every continuous function $f \in C(M,\R)$
\begin{equation}\label{weakracine}
\int_M f(s(x))\sqrt{\on{Jac}(s)}^2 \ud\on{vol}(x) = \int_M f(x) \ud \on{vol}(x)\,.
\end{equation}
\end{definition}
%For the reference volume measure we denote  $\sqrt{\on{Jac_{\on{vol}}}(s)}$ by  $\sqrt{\on{Jac}(s)}$.
%The product of $ (\varphi_1,\lambda_1)$,$(\varphi_2,\lambda_2)$ is defined by
%\begin{equation}
%(\varphi_1,\lambda_1) \cdot (\varphi_2,\lambda_2) = (\varphi_1 \circ \varphi_2,  (\lambda_1 \circ \varphi_2)  \lambda_2 )
%\end{equation}

%Obviously, $\autgc_{\on{vol}}(\mathcal{C}(M))$ contains all the natural lifts (Definition \ref{Th:NaturalLift}) of $\Diff(M)$.


\begin{theorem}[Polar factorization]\label{Th:polardecompo}
%Let $\rho_0$ be an absolute continuous admissible measure. 
Let $(\phi,\lambda) \in \autgc (\mathcal{C}(M))$ be an element of the generalized automorphism group of the half-densities bundle such that $\rho_1=\pi_0\left[(\phi,\lambda),\on{vol} \right]$ is an absolute continuous admissible measure. Then, there exists a unique minimizer, characterized by a $c$-convex function $z_0$, to the Monge formulation \eqref{Eq:MongeFormulation} between $\on{vol} $ and $\rho_1$ and there exists a unique measure preserving generalized automorphism $(s, \sqrt{\on{Jac}(s)}) \in \isog (\mathcal{C}(M))$ such that $\on{vol} $ a.e. 
%\begin{equation}
%(\phi,\lambda) = \exp^{\mathcal{C}(M)}(\nabla (r^2z_0) ) \circ (s,\sqrt{\on{Jac}(s)})\,,
%\end{equation}
\begin{equation}
(\phi,\lambda) = \exp^{\mathcal{C}(M)}\left(-\frac12 \nabla p_{z_0}, -p_{z_0} \right) \circ (s,\sqrt{\on{Jac}(s)})\,
\end{equation}
or equivalently
\begin{equation}
(\phi,\lambda) =\left(\varphi,  e^{-z_0} \sqrt{1 + \| \nabla z_0 \|^2} \right)   \cdot (s,\sqrt{\on{Jac}(s)})\,,
\end{equation}
where $p_{z_0}=e^{z_0}-1$ and 
\begin{equation}
\varphi(x) = \exp^{M}_x\left(-\arctan\left(\frac{1}{2} \|\nabla z_0(x) \| \right) \frac{\nabla z_0(x)}{\|\nabla z_0(x)\|}\right)\,.
\end{equation}
%Note that the notation $(s,\sqrt{\on{Jac}(s)})$ has the following weak sense: for every continuous function $f \in C(M,\R)$,
%\begin{equation}
%\int_M f(s(x))\on{Jac}(s)(x) \ud \rho_0(x) = \int_M f(x) \ud \rho_0(x)\,.
%\end{equation}
%\todofx{Il faut définir cet objet, la fermeture de l'ensemble des applications qui préservent la forme volume avant le théorème}
%\begin{equation}
%(\phi,\lambda) =\left(\varphi_{z_0},  \lambda_{z_0} \right)   \cdot (s,\sqrt{\on{Jac}(s)})\,.
%\end{equation}
%\begin{equation}
%(\phi,\lambda) =\left(\exp^{M}_x\left(\arctan\left(\frac{1}{2} |\nabla z | \right) \frac{\nabla z(x)}{|\nabla z(x)|}\right),  e^{z_0} \sqrt{1 + \| \nabla z_0(x) \|^2} \right)   \cdot (s,\sqrt{\on{Jac}(s)})\,.
%\end{equation}
Moreover $(s, \sqrt{\on{Jac}(s)})$ is the unique  $L^2(M,\mathcal{C}(M))$  projection of $ (\phi,\lambda)$ onto $\isog (\mathcal{C}(M))$.

\end{theorem}

We also state a more intrinsic formulation of the theorem.


\begin{corollary}
Denote by $\Mes^1(\mathcal{C}(M)))^{\R_+^*}$ the space of mesurable and approximate differentiable functions $f:\mathcal{C}(M) \mapsto \R$ that satisfy $f(x, r) = r^2 f(x,1)$ for any $r \in \R_+^*$.
Under the hypothesis of Theorem \ref{Th:PolarFactorisationStep},
there exists a unique couple $\left((s,\sqrt{\on{Jac}(s)}), \Psi_p \right) \in \isog \times \Mes^1(\mathcal{C}(M)))^{\R_+^*} $ such that
\begin{equation}
(\phi,\lambda) = \exp^{\mathcal{C}(M)}(-\nabla \Psi_p) \circ (s,\sqrt{\on{Jac}(s)})\,,
\end{equation}
where $\Psi_p(x,r) = r^2 p(x)$.
\end{corollary}
%Again, remark that if $s$ is smooth enough, $(s,\sqrt{\on{Jac}(s)})$ is the natural lift (see Definition \ref{Th:NaturalLift}) of $s$ in $\on{Aut}(\mathcal{C}(M))$.


\begin{proof}[Proof of Theorem \ref{Th:polardecompo}]
We denote $\rho_0=\on{vol}$ and $\rho_1= \pi_0\left[(\phi,\lambda),\rho_0\right]$. Let $(z_0,z_1)$ be a solution of $\on{WF}^2(\rho_0,\rho_1)$ and $\gamma$ be an optimal unbalanced transport plan. By symmetry, $(z_1,z_0)$ is a solution of $\on{WF}^2(\rho_1,\rho_0)$ and $\gamma^t$ is an optimal unbalanced transport plan. Let finally $(\varphi_0,\lambda_0)$ and $(\varphi_1,\lambda_1)$ be the two transport couples given by application of Proposition \ref{prop:approx}  to $(\rho_0,\rho_1)$ and $(\rho_1,\rho_0)$. We divide the proof into four small steps. We also denote $\on{dom}(f)$ the domain of definition of the function $f$.\\

{\bf Step 1: $ \varphi_0 $ and $\varphi_1 $ are inverse maps.}
On $U=\varphi_0^{-1}(\on{dom}{\tilde \nabla z_1})\cap \on{dom}(\tilde \nabla z_0)$ which has full $\gamma_0$ and therefore $\rho_0$ measure (we use here the admissible condition to say that $\gamma_0$ and $\rho_0$ have the same support), we have
$$
z_0(x)+z_1(\varphi_0(x))=c(x,\varphi_0(x))
$$
and thus 
 $ \varphi_1 (\varphi_0(x))=x$.  Similarly, it holds $ \varphi_0 (\varphi_1(y))=y$ on $V=\varphi_1^{-1}(\on{dom}{\nabla z_0})\cap \on{dom}(\nabla z_1)$ which has full $\rho_1$ measure.\\
 
 {\bf Step 2: $ (\varphi_0,\lambda_0)$ and $ (\varphi_1,\lambda_1) $ are inverse in $ \autgc$.}
 From Step 1, $\rho_1$ a.e. it holds $ \varphi_0 (\varphi_1(y))=y$. Thus,  $\rho_1$ a.e.
 $$
 (\varphi_0,\lambda_0) \cdot (\varphi_1,\lambda_1) = (\varphi_0\circ \varphi_1 ,\lambda_0 \circ \varphi_1  \lambda_1) = (\on{Id}, (\lambda_0 \circ \varphi_1) \lambda_1) \,.
 $$
Moreover by \eqref{Eq:MAEquation} of Proposition \ref{Th:PolarFactorisationStep} applied twice
\begin{align*}
\pi \left[ (\varphi_0,\lambda_0) \cdot (\varphi_1,\lambda_1), \rho_1 \right]=  \pi \left[ (\varphi_0,\lambda_0),  \pi \left[(\varphi_1,\lambda_1), \rho_1  \right] \right]   =  \pi  \left[ (\varphi_0,\lambda_0),\rho_0 \right]= \rho_1\,.
\end{align*}
It implies that 
$$ \pi \left[  (\on{Id}, (\lambda_0 \circ \varphi_1) \lambda_1) , \rho_1 \right]= \pi \left[ (\varphi_0,\lambda_0) \cdot (\varphi_1,\lambda_1), \rho_1 \right]=  \rho_1 \,.$$
In other words, we have $\rho_1$ a.e. $ (\lambda_0 \circ \varphi_1) \lambda_1=1$ and $\rho_1$ a.e.
$$
 (\varphi_0,\lambda_0) \cdot (\varphi_1,\lambda_1) = (\on{Id},1) \,.
$$
  
 {\bf Step 3: polar factorization.}
 Let $(s,\lambda_s)= (\varphi_1,\lambda_1) \cdot (\phi,\lambda)  = (\varphi_1 \circ \phi ,\lambda_1\circ \phi  \lambda ) $. By construction, one has
 \begin{align*}
\pi \left[ (s,\lambda_s), \rho_0 \right]=  \pi \left[ (\varphi_1,\lambda_1) \cdot (\phi,\lambda), \rho_0 \right] =  \pi \left[ (\varphi_1,\lambda_1),  \pi \left[ (\phi,\lambda),\rho_0  \right] \right]   =  \pi  \left[ (\varphi_1,\lambda_1),\rho_1 \right]= \rho_0\,.
\end{align*}
Therefore, $(s,\lambda_s)$ belongs to $\isog$ and $\lambda_s=\sqrt{\on{Jac}(s)} $ holds in the weak sense \eqref{weakracine}. Thus 
$$
(\phi,\lambda) = (\on{Id},1)\cdot(\phi,\lambda) = (\varphi_0,\lambda_0) \cdot   (\varphi_1,\lambda_1) \cdot (\phi,\lambda) = (\varphi_0,\lambda_0) \cdot (s, \sqrt{\on{Jac}(s)} )\,.
$$
It proves the polar factorization. 

{\bf Step 4: Uniqueness.}
%We first observe that any pair of c-convexe potentials $(\bar z_0, \bar z_1) $ is optimal for $\on{WF(\rho_0,  \left[ (\varphi_0,\lambda_0),\rho_0 \right] )}$.
The pair of c-convex potentials $(z_0,z_1)$ is optimal for $\on{WF(\rho_0,  \left[ (\varphi_0,\lambda_0),\rho_0 \right] )} =  \on{WF(\rho_0,  \rho_1 )}$ and therefore by Proposition \ref{Th:PolarFactorisationStep}, $ z_i $ are unique $\rho_i$ a.e..
%By  the potential $z_0$ associated the couple $  (\varphi_i,\lambda_i)$ are unique $\rho_i$ a.e.
We deduce that the projection  $(s,\sqrt{\on{Jac}(s)})= (\varphi_1,\lambda_1) \cdot (\phi,\lambda) $ is also unique $\rho_0$ a.e.. Indeed the positivity of $\lambda$ implies that $\on{Supp}(\lambda^2\rho_0)=\on{Supp}( \rho_0)$, thus $\phi$ maps $ \on{Supp}(\rho_0)$ onto $\on{Supp}(\rho_1)$ and the uniqueness of $\varphi_1$ and $\lambda_1$, $\rho_1$ a.e.,
implies the uniqueness of $s$ and $\sqrt{\on{Jac}(s)}$, $\rho_0$ a.e..
To prove that   $(s,\sqrt{\on{Jac}(s)}) $ is the $L^2(M,\mathcal{C}(M))$  projection of $ (\phi,\lambda)$ onto $\isog (\mathcal{C}(M))$, we observe  %for any $(\sigma,\lambda_{\sigma}) \in \isog (\mathcal{C}(M)) $: 
\begin{align*}
\inf_{(\sigma,\sqrt{\on{Jac}(\sigma)} ) \in \isog (\mathcal{C}(M)) } &  \left \| (\phi,\lambda) - (\sigma,\sqrt{\on{Jac}(\sigma)} ) \right \|^2_{L^2(\rho_0)} \geq \on{WF}^2(\rho_0, \rho_1) \\
&%= \left \| (\varphi_1,\lambda_1) - (\Id,1) \right \|^2_{L^2(\rho_1)} 
=  \left \| (\varphi_0,\lambda_0) - (\Id,1) \right \|^2_{L^2(\rho_0)} \\ 
& = \left \| (\varphi_0,\lambda_0)\cdot (s,\sqrt{\on{Jac}(s)} ) - (s,\sqrt{\on{Jac}(s)} ) \right \|^2_{L^2(\rho_0)}=  \left \| (\phi,\lambda) - (s,\sqrt{\on{Jac}(s)} ) \right \|^2_{L^2(\rho_0)}\,,
\end{align*}
which gives the result.

%\todofx{L'unicité n'est pas prouvée}
% \overline{ \on{Aut}(\mathcal{C}(M))} = \on{S}\overline{ \Diff(M) \ltimes_\Psi \Lambda_{1/2}(M) }
\end{proof}

This polar factorization could probably be understood, under minor verifications, in the framework of abstract polar factorization of Brenier \cite{Brenier1991}. As in the case of classical optimal transport, Theorem \ref{Th:polardecompo} could be extended, for example, to any 
admissible $\rho_1$ without the absolute continuity assumption. In this case, one looses uniqueness of the measure preserving generalized automorphism $(s, \sqrt{\on{Jac}(s)})$. An other direction is to project on the subset of $\autgc(\mathcal{C}(M))$: 
$$
\isogh (\mathcal{C}(M)) = \left\{ \left(s,\lambda \right) \in \autgc(\mathcal{C}(M)) \, \middle| \, \pi\left((s,\lambda),\rho_0\right)=\mu_0  \right\}\,,
$$
in the spirit of \cite[Theorem 3.15]{VillaniTOT}. The proof is similar to the one given above.
% Similarly to the Incompressible Euler equation the Geodesic of $\isogh (\mathcal{C}(M))$ would leads to another class of Camassa-Holm equations with different measure preserving constraint. The method developed in this paper can be easily adapted to this situation. 
This polar factorization also yields by linearization an Helmholtz decomposition of velocity vector fields \comment{given as the sum of an element in the horizontal space and an element the vertical space, see Propositions \ref{Th:RiemannianSubmersion} and \ref{HorizontalLiftFormulation}  }% We will not go further in these directions and leave it for future works. 


%
%{\color{red} Preuve 1 avec les potentiels\\
%\begin{lemma}[super-differentiability]
%%\begin{itemize}
%%\item Let $y \in M$, the function $f$ defined on $M$ by $f(x)= -\ln(\cos^2(d (x,y ))$ is super-differentiable.
%%\item Let $y \in M $, the function $g$ defined on $M$ by $g(x)= -\ln(\cos^2(d^2_{\frac{\pi}{2}}(x,y))$ is super-differentiable on $B_d{(y,\frac{\pi}{2})}$.
%%\end{itemize}
% Let $y \in M $, the function $g$ defined on $M$ by $g(x)= c(x,y)$ is super-differentiable on $B_{y}(\frac{\pi}{2})$.
%\end{lemma}
%\begin{proof}
%The function  $ d^2(\cdot,y)$ is super-differentiable see \cite[Proposition 6]{McCann2001} for instance. Therefore $d^2_{\frac{\pi}{2}}(\cdot,y)=\left(d(x,y)\wedge {(\pi / 2)}\right)$ %\on{inf}\left(d^2(\cdot,y), \frac{\pi}{2}\right)$
%is also supper-differentiable. Since the function $-\log\left(\cos^2(\sqrt{2\cdot}\right))$ is $C^1$ on $[0,\frac{\pi}{2}[$ 
%the function $g$ is super-differentiable on $B_{y}(\frac{\pi}{2})$ as the combinaison of an increasing $C^1$ function and the super-differentiable function  $ d^2_{{\pi}/{2}}(\cdot,y)$ see \cite[Lemma 5]{McCann2001}. 
%\end{proof}
%\begin{proposition}[Approximate differentiability]
%Let $\rho_1$, $\rho_2$ be two measures and $(z_1, z_2)$ be the optimal potentials for $\on{WF}^2(\rho_1,\rho_2)$.  \todofx{Replace $\L$ with $\on{vol}$}
%Suppose that $\rho_1$ and $\rho_2$ are admissible and $\rho_1 << \on{vol}$, then $z_1$ is approximate differentiable on $Supp(\rho_1)$. Moreover 
%\begin{equation}\label{eq:unicitetransport}
%\tilde \nabla z_{1} (\bar x) = 2 \tan (|\zeta|)   \frac{ \zeta }{| \zeta| }. \quad a.e.
%\end{equation}
%\end{proposition}
%\begin{proof}
%The proof is an adaptation of \cite[Theorem 6.7]{LieroMielkeSavareLong} using arguments in \cite{McCann2001,villani2008optimal}. %The two main difficulties are the fact that the cost may be infinite 
%%and we work on a Riemannian manifold. 
%Let $(z_1, z_2)$ be the optimal potentials for $\on{WF}^2(\rho_1,\rho_2)$ and $\gamma$ the optimal potential \cite[Theorem 6.3]{LieroMielkeSavareLong}.
%Since $\rho_1$ and $\rho_2$ are admissible then $\Pi_1(\gamma)=\rho_1$ and $\Pi_2(\gamma)=\rho_2$. Therefore there exists Borel sets $A_1\subset \on{Supp}(\rho_1) $ and $ A_2 \subset \on{Supp}(\rho_2)$ with $\rho_1(M\setminus A_1)=\rho_2(M\setminus A_2)=0  $ such that 
%\begin{align*}
% %& z_1(x)+z_2(y) \leq -\ln(\cos^2(d^2_{\frac{\pi}{2}}(x,y))  &  \on{in  }  A_1 \times A_2     \\
% & z_1(x)+z_2(y) \leq c(x,y)  &  \on{in  }  A_1 \times A_2     \\
% & z_1(x)+z_2(y) = c(x,y) &   \gamma-\on{a.e.   } \on{in  } A_1 \times A_2
%\end{align*}
%
%To construct the set of approximate differentiability let 
%$$
%s_{1,n} = \inf_{y\in A_{2,n}} c(x,y) -z_2(y)
%$$
%%$$
%%A_{2,n} = \left \{  y\in M \middle \| \sigma_2(y) \geq 1/n    \right \}
%%$$
%$$
%s_{2,n} = \left \{  y\in M \, ;\, z_2(y) \leq  n    \right \},
%$$
%and consider the function 
%$$
%z_{1,n}= \inf_{y\in A_{2,n}} c(x,y) -z_2(y)
%$$
%%{\color{red}  Ici on utilise deja Savare pour dire que on a l'existecence d'un y otpimal pour $\gamma_i$ et donc $\mu_i$ presque tout x, c'est truc de gagne deja par rapport a McCAnn.   Ensuite la preuve est 1 on coupe pour avoir des fonctions differentiable en n, sur un ensemble gras.}
%
%
%%Let $\sigma_i= -\log(z_i)$, the constraint reads
%%$$
%%\sigma_1(x) \sigma_2(y) \geq \cos^2( d_{\frac{\pi}{2}}(x,y ) ), \quad x,y \in M \times M. 
%%$$
%%and 
%%\begin{equation}\label{cconvex}
%%\sigma_1=\sup_{y\in M}  \cos^2( d_{\frac{\pi}{2}}(x,y ) )/ \sigma_2(y).
%%\end{equation}
%%
%%We define the set $A_{2,n}$ by 
%%$$
%%A_{2,n} = \left \{  y\in M \middle \| \sigma_2(y) \geq 1/n    \right \}
%%$$
%%and the function 
%%$$\sigma_{1,n} = \sup_{y\in A_{2,n}}  \cos^2( d_{\frac{\pi}{2}}^2(x,y ) )/ \sigma_2(y).$$
%By construction $\sigma_{1,n} $ is bounded Lipschitz and thus differentiable  $\on{vol}$ a.e.  
%Since  $ \sigma_1 \geq \sigma_{1,n}$ the set $A_{1,n} =\left\{  x \in M \,;\, \sigma_1(x) = \sigma_{1,n}(x)  \right\} $ are increasing
%and $ \cap_{n=1}^{\infty} (X\setminus A_{1,n})$ is $\on{vol}$ negligible. 
%Let  $$A'_{1,n} =\bigcap \left\{  x \in A_{1,n}  \, ; \,\lim\limits_{r\to 0} \frac{\on{vol}(B(x,r)\cap A_{1,n} )}{\on{vol}(B(x,r))}=1  \right\} $$
%be the set of points with density 1. Remark that  $ \cap_{n=1}^{\infty} (X\setminus A'_{1,n})$ is $\on{vol}$ negligible.
%
%Let $(\bar x,\bar y)\in A'_{1,n}\times A_{2,n}$ such that 
%$$
%\sigma_{2,n}( \bar y) \sigma_{1,n}(\bar x) = \cos^2( d_{\frac{\pi}{2}}( \bar x, \bar y) ).
%$$
%For all $x \in M$ 
%$$
%\sigma_{2}(y)  \geq \cos^2( d_{\frac{\pi}{2}}(x,\bar y) )/ \sigma_{1,n}(x).
%$$
%In particular $0 \in \nabla_{\bar x }^{-} ( \cos^2( d_{\frac{\pi}{2}} (\cdot,\bar y) )/ \sigma_{2}(\bar y))$ it implies 
%that $d^2(\cdot,y)$ is sub-differentiable at $\bar x$ since it is also super-differentiable it is differentiable and 
%\begin{align*}
%0&= \nabla ( \cos^2\left( \sqrt{2} \sqrt {\frac12 d^2_{\frac{\pi}{2}} (\bar x,\bar y) }) \right) /  \sigma_{1,n}(x) - \cos^2( d_{\frac{\pi}{2}} (\bar x ,\bar y))  \nabla \sigma_{1,n}(\bar x)/  \sigma^2_{1,n}(x)\\
%&= 2 \sqrt{2} \tan( d_{\frac{\pi}{2}} (\bar x ,\bar y)) \frac{\sqrt{2}}{2_{\frac{\pi}{2}} (\bar x ,\bar y)}\nabla ( {\frac12 d^2_{\frac{\pi}{2}} (\bar x,\bar y) }) -   \nabla \ln  \sigma_{1,n} (\bar x) \\
%\end{align*}
%Let $\zeta  \in T_{\bar x} M$ be the unique vector such that $\bar y = \exp^{M}_{\bar x}(\zeta)$ we have 
%$$
%\tilde \nabla \ln  \sigma_{1} (\bar x)= \nabla \ln  \sigma_{1,n} (\bar x) = -2 \tan (|\zeta|)   \frac{ \zeta }{| \zeta| }. 
%$$
%\end{proof}}
%{\color{red} Preuve 2 avec les densites}

















